RGD: Multi-LLM Based Agent Debugger via Refinement and Generation Guidance

Large Language Models (LLMs) have shown incredible potential in code generation tasks, and recent research in prompt engineering have enhanced LLMs' understanding of textual information. However, ensuring the accuracy of generated code often requires extensive testing and validation by programmers. While LLMs can typically generate code based on task descriptions, their accuracy remains limited, especially for complex tasks that require a deeper understanding of both the problem statement and the code generation process. This limitation is primarily due to the LLMs' need to simultaneously comprehend text and generate syntactically and semantically correct code, without having the capability to automatically refine the code. In real-world software development, programmers rarely produce flawless code in a single attempt based on the task description alone, they rely on iterative feedback and debugging to refine their programs. Inspired by this process, we introduce a novel architecture of LLM-based agents for code generation and automatic debugging: Refinement and Guidance Debugging (RGD). The RGD framework is a multi-LLM-based agent debugger that leverages three distinct LLM agents-Guide Agent, Debug Agent, and Feedback Agent. RGD decomposes the code generation task into multiple steps, ensuring a clearer workflow and enabling iterative code refinement based on self-reflection and feedback. Experimental results demonstrate that RGD exhibits remarkable code generation capabilities, achieving state-of-the-art performance with a 9.8% improvement on the HumanEval dataset and a 16.2% improvement on the MBPP dataset compared to the state-of-the-art approaches and traditional direct prompting approaches. We highlight the effectiveness of the RGD framework in enhancing LLMs' ability to generate and refine code autonomously.

==> page/discussion.tex <==
\section{Limitation\label{cha:discussion}}
% For the limitations of RGD, the primary limitation currently is that our system does not handle input-output test cases comprehensively enough to cover all situations. For example, in the APPS dataset, we need to handle the competition-level test sets specially to be able to perform the tests. Additionally, if the number of test cases is too large, such as with some samples in the MBPP-ET dataset, it can lead to excessive token usage and a high likelihood of failing to understand all the content since a significant portion of the prompt consists of test cases. Our current solution is to randomly select five test cases as input for the Feedback Agent if the number exceeds five. Another limitation is that code fixes are highly dependent on the results of failure analysis; the code is largely repaired based on the information provided in the analysis. Therefore, if the response generated by the Feedback Agent is of poor quality, it could steer the debugging in an undesirable direction.

%In future work, conducting more experiments with different models, especially open-source large models, will provide deeper insights and help identify potential limitations of our framework. Additionally, introducing more benchmarks for testing will further evaluate its effectiveness.
